When could NISQ algorithms start to create value in discrete manufacturing ?

Are quantum advantages in discrete manufacturing achievable in the near term? As manufacturing-relevant NISQ algorithms, we identified Quantum Annealing (QA) and the Quantum Approximate Optimization Algorithm (QAOA) for combinatorial optimization as well as Derivative Quantum Circuits (DQC) for solving non-linear PDEs. While there is evidence for QAOA's outperformance, this requires post-NISQ circuit depths. In the case of QA, there is up to now no unquestionable evidence for advantage compared to classical computation. Yet different protocols could lead to finding such instances. Together with a well-chosen quantum feature map, DQC are a promising concept. Further investigations for higher dimensional problems and improvements in training could follow.

==> chapters/abbreviations.tex <==
\makeglossaries

\newacronym{qa}{QA}{quantum annealing}

\newacronym{qaoa}{QAOA}{quantum approximate optimization algorithm}

\newacronym{dqc}{DQC}{differentiable quantum circuit or equivalent derivative quantum circuit}

\newacronym{qsvm}{QSVM}{quantum support vector machine}

\newacronym{nisq}{NISQ}{noisy intermediate-scale quantum}

\newacronym{qubo}{QUBO}{Quadratic unconstrained binary optimization}

\newacronym{hhl}{HHL}{Harrow Hassidim Lloyd algorithm or quantum algorithm for linear systems of equations}

\newacronym{cop}{COP}{combinatorical optimization problem}

\newacronym{jssp}{JSSP}{job shop scheduling problem}

\newacronym{aqc}{ACQ}{adiabatic quantum computation}

\newacronym{qc}{QC}{quantum computation}

\newacronym{sdp}{SDP}{semidefinite programming}

\newacronym{pde}{PDE}{partial differential equation}

\newacronym{fem}{FEM}{finite element methods}

\newacronym{qram}{QRAM}{quantum random access memory}

\newacronym{qec}{QEC}{quantum error correction}

\newacronym{vqa}{VQA}{variational quantum algorithms}

\newacronym{vqc}{VQC}{variational quantum circuit}

\newacronym{ml}{ML}{machine learning}

\newacronym{fvm}{FVM}{finite volume method}

\newacronym{ph}{PH}{polynominal hierarchy}

\newacronym{ftqc}{FTQC}{fault-tolerant quantum computing}

==> chapters/backup.tex <==
\clearpage

\section{Assessment of NISQ algorithms }\label{sec:assessment}
In this section, we complete the evaluation of the algorithms regarding the criteria in \ref{chap:3}.

\textbf{Universality need}: Among the identified algorithms, QA can be realised in a quantum annealer while the other algorithms involve gate operations and require a gate-based QC. This leads to a temporal advantage for the realisation of practical application via QA.

\textbf{Performance advantages and corresponding hardware requirements}:
\begin{itemize}
    \item QA can lead to faster computations for problems tailored to the given QA protocol already now. In the future, multiple QA protocols and suitable combinatorial optimization problems have to be investigated to maximally benefit from QA. Yet there is a non-zero probability that a random optimization problem is also amenable to a speed-up through QA. 
    \item QAOA with depth p > 11 and a few hundred qubits could find better solutions for meaningful applications. This could be implemented after 2025 (see section \ref{sec:quantum hardware platforms}). Especially highly complex problems are suited to be addressed. 
    \item DQC are not been extensively studied so far. Yet the results for prototype problems are promising. As plenty of operations are required, the applicability of real-world problems would be improved if coherence time is enlarged. Furthermore, for each PDE individually feature maps have to be constructed within that framework.
\end{itemize}

\textbf{Generality}: We estimate that more problems of the addressed problem type through QAOA and DCQ would profit than in the case of QA. %to apply to more manufacturing use cases than QSVM.
We estimate that QA for certain problems can lead to a significant speed-up already nowadays. Although it may not be superior to classical computation for a majority of COP, it could become for all problems an increasingly competitive option. 
We assess the initial time of value creation through QAOA after 2025 for a broad variety of COP. Finally, DQC could also create value for well-studied PDEs. The prerequisite is that suitable feature maps are developed and a sufficient depth is reachable.

%NISQ (3-5), late NISQ (5-10), post NISQ +10  through hardware roadmaps. 



%This influences the near term beneficence of the algorithms. 




%\section{Overview of computational intensive problems in discrete manufacturing} 
%-> value 
%\marginnote{Classify after problem domain (optimization, ML, ...) }
%\section{Landscape of quantum algorithms}

%solving open challenges
%\section{Optimization}%Problem domain



%\section{Hardware platforms and criteria to assess time typing}
%NISQ  simulator, annealer, ising machine, ... 
%for the use cases:
%\subsection{Quantum Annealer}
%simulator, QA, ising machine
%\subsection{Universal gate-based quantum computer}
% \subsubsection{}

%Superconducting, Ion Trapped, Photonics

%-> energy efficency 
%-> expenses

%\section{Criteria to assess value typing}




%\subsection{Grover}
%\marginnote{algos, speed-up, hardware requirements, time}
%\underline{Lowdepth Grover}

%\section{VQE}


%\paragraph{Example: Optimization of robot trajectory planning @BMW}
%\paragraph{Example: Mix Sigma with quantum-inspired QA @TLabs\&Fujitsu}
%SDP
%\section{Simulation}
%\subsection{Hamitonian simulation}
%\subsection{VQE}
%\section{Linear Algebra}
%\section{VQLS}
%\subsection{HHL}

%\subsection{Example: Tool modelling with HHL algorithm @TRUMPF}
%QUASIM 
%\subsection{Recommendation Systems}
%ML
%\section{Fourier Transformation}
%\subsection{Shor}
%\section{Machine learning}


%\subsection{Example: Quality control with quantum classification algorithms @Bosch}
%\subsection{Reeinforcement learning}
%\subsection{Neural Nets}
%functunality and implications for business


%\section{Quantum business experiments}
%Applications of quantum computing in discrete manufacturing
%Current quantum computing applications in the manufacturing industry


%BMW AWS
%\section{ML with Siemens for Health Cear Device}

%\section{Vehicle routing}
%supply chain optimization
%Accenture Quantum Business Experiments
%https://www.youtube.com/watch?v=eOMMkwOnGbY&ab_channel=QCWare
%\subsection{Automated Scheduling}
%in the Healthcare Sector

%\subsection{Waste Reduction }
%https://www.youtube.com/watch?v=3a6J34SVE_I&ab_channel=BitkomEvents
%https://www.quantum-summit.com/programme#nid-515

%\section{Overview of met challenges}




%\section{Application area in discrete manufacturing}\label{sec:application domain size}

A speed-up is related to the required amount of quantum operations. Assuming one unit of time per operation, the fewer operations are needed the faster the computation. Increasing the number of operations can improve the precision of the result but will take longer and elevate the device requirements for coherence time. 
In the cases of variational quantum circuits, increasing the number of operations can lead to the need for fewer qubits. 
Also, increasing the number of qubits may allow encoding higher value problems but is realisable even further in the future. 
The whole algorithm architecture (width and depth) will have an impact on the quality of the result. 
Moreover, the problem itself poses demands on the algorithmic architecture. The use case itself influences the realisation time heavily through the geometry of the problem and the problem size.  

The relevant problem domains in discrete manufacturing that are amenable to the identified NISQ algorithms are optimization and numeric engineering simulation.
According to McKinsey the first value creation in the discrete manufacturing industry will occur in the automotive industry as an innovation driver \cite{McK:use_cases}. Therefore we will briefly discuss the relevance of the problem domains for this industry separately. 
%McKinsey estimates the value potential of optimization applications (e.g. robot path planning and job scheduling) higher than those for machine learning (e.g. autonomous driving).
The importance of optimization for automotive manufacturing is due to the rising number of vehicle configurations. Different configurations lead to different processes. Therefore the search for optimal job scheduling is important. Numeric engineering simulations are relevant for vehicle design. 
Both problem types are ubiquitous in manufacturing \cite{a:automotive}.
%ML-based near-term quantum use cases in the automotive industry are automatic optical inspection and predictive maintenance in the frame of autonomous driving. Furthermore, the identification of causes of rare failures manufacturing processes is an important ML task \cite{bova2021commercial}. Although failure happen rarely, their occurence causes huge costs.
%According to McKinsey there are currently less quantum machine learning applications that are proven to work than in the other problem domains. Consequently this is an inicator to assess QSVM less general than the other algorithms although there is a great potential to develop more ML use cases and advance them via QC to improve manufacturing processes.
%TODO  Expert needed

%Considering the quantum use cases in the automotive industry the application frequency and domain size of optimization and numeric engineering simulation is greater than for machine learning. 
%Having that said, there is a huge potential to develop more ML use cases and advance them via QC to improve manufacturing processes.


%This latter fact leads to a lower value estimate. Regarding the use cases in \ref{sec:usecases} we also recoginze the multitude of optimization applications. On the other side the optimization algorithms are invented earlier than the algorithms for solving PDE's.
 %but not as near-term feasiable due to the high parameter space in real world problems, whereas in optimization problems subproblems can be easily formulared and first solved to create a composite solution.
%BCG reckon the value creation potential of quantum computation the the field of simulation in the automotive and aerospace industrie overall higher than in the field of optimization. Machine learning is estimated the lowest in value creation overall\cite{bcg}.

%As noted in section \ref{sec:discrete_manufacturing} in general all three problem types are omnipresent in the manufacturing context.% TODO qutac nachlesen

Now we also can use the quantum use case overview in \ref{sec:usecases} to draw further conclusions about the criterion generality. The mentioned numbers are illustrated in figure \ref{fig:data_generality}.
\begin{itemize}
    \item QA and QAOA: In the quantum use cases there is a majority in the field of optimization. Seven out of eleven use cases were in this regime. QAOQ and QA are known since respectively 2014 and 1989.
    \item DQC: Numeric engineering simulation was addressed in only three out of eleven industry use cases. The DQC for solving non-linear PDE's algorithm was published not long ago in 2021. Moreover, for non-linear differential equation solvers, available quantum protocols are sparse and the field is only starting to grow. The time disadvantage is one factor for its underrepresentation.
   % \item QSVM: QSVM is known since 2014 and we found only one quantum use case in discrete manufacturing. Even though the use cases can not claim representativity with certainty, this can be an indicator that fewer use cases are developed to date as in the other two fields.
\end{itemize}

\begin{figure}[h]
 	\input{generality.tikz}
	\caption{Data for the generality assessment based on the use case overview in \ref{sec:usecases}. On the x-Axis, the number of quantum use cases in discrete manufacturing from section \ref{sec:usecases} the algorithm applies to is plotted. On the y-Axis, we draw the years that passed since the publication of the algorithm.}
	\label{fig:data_generality}
\end{figure}


%Thus we estimate the relative value potential of optimization and numeric engineering simulation higher than those for machine learning applications in the early stage. 
%We conclude that regarding generality we estimate QA, QAOA and DQC to be assessed relatively higher than QSVM in the early stage.

For our investigation, the applicability is only necessary but not sufficient. For value creation, a performance advantage is also required. QA may not be advantageous to its classical counterpart in a part of the cases as discussed in \ref{qa} unless problem-specific protocols are developed. Therefore we estimate the generality a bit lower than for the other algorithms. Having said that, QA could be competitive with classical approaches in all cases.  
We conclude that regarding generality we estimate QAOA and DQC to be assessed higher than QA.


==> chapters/frontmatter/abstract.tex <==

\begin{abstract}
   %discrete manufacturing, automotive industry
   %job scheuduling
 Quantum algorithms outperform classical algorithms at specific computational tasks. As a result, quantum computing has an accelerating or even disruptive potential for computational challenges in the discrete manufacturing industry. 
  Yet the required maturity of quantum hardware to solve real-world problems is not reached. 
 %  Untractable computationally-dependent
 %  business problems could be approached and 
 %  existing solutions could be accelerated s.t. they meet the demands of companies. 
%Major discrete manufacturing companies are evaluating which business problems are amenable via quantum algorithms. 
%In the next two years quantum algorithms in the domains of machine learning, optimization and modelling are estimated to create the highest revenues \cite{hyperion:vid}.  

It remains unknown whether during the \acrfull{nisq} era, which we claim to transition to \acrfull{ftqc} after 2016, a quantum advantage for practical problems is possible.
%when and with which revenue real problems will start to be addressable. 
For more clarity, we investigate NISQ algorithms underlying manufacturing applications. Then the hardware requirements are explored for cases with evidence of performance advantage through NISQ algorithm usage. 

 %Therefore first, we identify \acrfull{nisq} quantum algorithms which are in current evaluation for discrete manufacturing applications. Second, we investigate their functionality and hardware requirements. Third, we assess the algorithms to compare the time of first value creation through the application of these algorithms.

We identified \acrfull{qa} and \acrfull{qaoa} for combinatorial optimization as well as \acrfull{dqc} for solving non-linear PDEs as manufacturing-relevant NISQ algorithms. Thereby we expect QA to start to create value in problems tailored to the QA protocol (e.h. highly complex) as soon as such problems and QA protocols are matched. Whereas, we estimate QAOA to enhance production scheduling and production processes broadly when over 22 operations are reliably implementable on a few hundred qubits. Given the quantum computer provider's roadmaps, this seems realisable after 2025. DQC is useful for product design by enabling faster engineering simulations. Thereby the feature maps have to be tailored to the PDE of interest and also here a higher coherence time of the quantum computer will be of use.
All over, we are confident that NISQ algorithms will create value in discrete manufacturing during the NISQ era if efforts for problem-specific adaptions are made. 
%While QA and QAOA could optimise production scheduling and production procescses further, DQC 

%Use cases for \acrshort{qa} and \acrshort{qaoa} include desgin optimization for sensor positions and mirror shapes in a vehicle as well as process optimization for matrix production, binary paint shop, robot trajetories and mix sigma.Binary classification for tensil test is a use case for \acrshort{qsvm}. Tensil test simulation can be achieved also through \acrshort{dqc}. 

%<more on results>
 %results 
%To contribute to more clearity we identify quantum algorithms which are in evaluation for discrete manufacturing industry applications and understand their implications for business. 
%In these problem domains we survey current quantum business experiments in discrete manufacturing and examine the underlying algorithms. 
%The complexity of the algorithm has implications for its value potential. The result (approximation/ exact solution) as well as the problem size has implications for the hardware requirements and therefore for the time of realisation. 
%The table summarizes the results:\\
%their usage including the mathematical model of the use cases, their speed up/ value est., their noise-tolerance, time est. .  


%We hope that through this typing near term use cases will be eaiser to identifiy, giving orientation for manufacturer's usage consideration of quantum technologies. 
   

   %According to Hyperion Research in 2021 over 40\% of companies worldwide have obstacles to solve computationally-dependent business problems and next to it many implemented solutions do not meet the demands of companies fully.
%   The thesis aims to systemize where to meet computational challenges in discrete manufacturing with quantum algorithms and elaborate their implications for business. 
   
  % We explore optimization, simulation and machine learning as highest revenue estimated problem domains so far (\cite{hyperion:vid}) and survey indursty use cases. To these use cases we match NISQ quantum algorithms to evaluate near term solutions for manufacturing problems. 
   

  % Finally we select a case that has a relative high impact on the business and can be realised in the near term.
  % The case namely is optimazation of <high value problem> through <NISQ Algo> that can be realised <time> 
   
\end{abstract}


==> tab/tab.tex <==

\begin{table}[]
    \centering
    \begin{tabular}{ccccc}
    \toprule
    \multicolumn{4}{c}{\bf time} \\
     \diagbox[]{criteria}{algorithm}  & QA & QAOA & DCQ & QSVM \\ 
     \midrule
    universality unnecessity & 1 & 0 & 0 & 0 \\
   % shallow operations &  &  &  & \\
    %feasable problem data size &  &  &  & \\\midrule
    %time score &  &  &  & \\
   %\toprule
    \multicolumn{4}{c}{\bf value}\\
      \diagbox[]{criteria}{algorithm}   & QA & QAOA & DCQ & QSVM \\ 
      \midrule
       generality  & 1 & 1 &  1 & 0 \\ 
    %   speed-up &  &  &  & \\
    %   accuracy &  &  &  & \\ \midrule
     %  value score &  &  &  & \\
    \bottomrule 
    \end{tabular}
    \caption{ Classification of the NISQ algorithms regarding the criteria universality and generality}
    \label{tab:my_label}
\end{table}



The problem data size is given in table \ref{tab:datasize} for the relevant cases.

\begin{table}[]
    \centering
    \begin{tabularx}{\textwidth}{p{3cm} X}
      \bf use case   & \bf problem data size \\\toprule
     noise minimization for vehicle design &  in the order of millions parameter \\\midrule
      binary paint shop & \\\midrule
      sensor position optimization & in the order of hundert allowed sensor postions\\\midrule
      tensil test & \\\midrule
      robot trajectory planning & 71 seams \\ \midrule
      wingbox optimisation & 6 structural parameters \\\midrule
      mix sigma & 90 possible configuarations \\\midrule
      nesting and scheduling optimization in sheet metal processing &  $P\cdot S \cdot C \cdot H$ where $P$ is the number of parts, $S$ is the number of metal sheets, $C$ is the number of cutting machines and $H$ is the horizon.
    In real planning applications, the number of parts can be hundreds, the number of sheets tens, the horizon (>makespan) hundreds, resulting in a need of hundreds of thousands of qubits. \ref{a:sheetmetal}\\\midrule
      realtime shop floor optimization& A matrix production is composed of multiple coupled processes. One process can contain <> data points, which is the order of needed qubits as the processes can be optimized separelty  \\ 
      \bottomrule
    \end{tabularx}
    \caption{Problem data size for quantum comutation use cases in discrete manufacturing}
    \label{tab:datasize}
\end{table}




\begin{table}
\begin{tabular}{p{8 cm} p{3 cm}}
\toprule
manufactured good & revenue in billion U.S. Dollars \\
\midrule
motor vehicles, trailers and semi-trailers &	630.73\\
machinery and equipment n.e.c. &	304.65\\
food products 	&236.02\\
chemicals and chemical products 	&202.30\\
fabricated metal products, except machinery and equipment 	&185.66\\
computer, electronic and optical products &	179.41\\
coke and refined petroleum products &	147.00\\
basic metals &	148.92\\
rubber and plastic products 	&138.01\\
basic pharmaceutical products and pharmaceutical preparations &	112.35\\
electrical equipment &	105.69\\
other transport equipment 	&98.70\\
other non-metallic mineral products &	64.02\\
other manufacturing &	58.66\\
paper and paper products &	54.71\\
wood and of products of wood and cork, except furniture, articles of straw and plaiting materials& 	33.06\\
beverages &	33.65\\
furniture &	29.99\\
tobacco products &	27.64\\
printing and reproduction of recorded media &	23.08\\
repair and installation of machinery and equipment& 	19.07\\
textiles &	17.19\\
wearing apparel &	12.99\\
leather and related products 	&5.87\\
\bottomrule
\end{tabular}
\caption{\label{tab:revbygood} Revenue obtained 2019 through manufacturing of goods in Germany. Source:  Eurostat}
\end{table}




\begin{table}[]
    \centering
    \begin{tabular}{c c}
    \toprule
      real data size & in the order of million data points \\
      used data size  & \\
        computation time sensitivity & \\
        \midrule
        value of good & \\
        computation frequency & \\
        results & proof of concept\\
        \bottomrule
        \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}




%\begin{adjustbox}{center}
%\begin{tabular}{*{4}{l}}
%\toprule
%    &\multicolumn{3}{c}{problem domains}\\
 %   \cmidrule(r){2-4}
 %    & optimization & modeling & machine learning \\
 %     \cmidrule{2-3} \cmidrule{3-4}
 %    problem class &  QUBO  & FEM  &  gradient calculation\\
 %    mathematical model & Ising spin model & operator inversion  & ?\\
  %   quantum algorithms & QAOA , QA & HHL & QSVC \\
 %    use cases& Mix sigma  & tool modeling & quality control  \\
 %    speed-up & heuristic & exponential & heuristic  \\
 %    hardware requirements & low, Annealer& medium& low\\
 %    realisation time & near term (3-5 years) & mid term (5-10 years)& low(3-5 years) \\
%\bottomrule     
%\end{tabular}
%\end{adjustbox}
%\begin{adjustbox}{center}




\begin{landscape}
  \begin{longtable}{p{\textheight / 20} p{\textheight / 5}  *{9}{p{\textheight / 10}}}
 domain & use case  & classical alternative  & problem frequency & value of good & computation time sensitivity & real problem data size & problem class & mathematical model & algorithm & results\\
 \toprule
 \endhead   
 \multicolumn{6}{c}{\bf VW}\\\\
 % Logistics &  Predicting and maximizing traffic flow:  Capacitated Vehicle Routing Problem (CVRP) modeled as multiple QUBO subproblems & real time  &  \href{https://www.microsoft.com/en-us/research/publication/t-drive-trajectory-data-sample/}{T-Drive trajectory data sample} with 15 million data points & QA & No \\
 design optimization & minimizing the wind noises on an external mirror of a vehicle, minimizing the noises through vibrations caused by the engine or different road conditions in a vehicle & FEM & medium & high& tolerant & in the order of millions &  ? & QUBO& QA & proof of concept \\
 optimization & binary paint shop & machine learning & medium & high & real-time & hunderts & ? & spin glas& \href{https://quantumai.google/cirq/experiments/qaoa/binary_paintshop}{QAOA} & advantage compared to classical heuristics\\
 \multicolumn{6}{c}{\bf BMW}\\\\
desgin optimization & sensor position optimization& & low & high & tolerant & order of 100 allowed sensor positions & MaxCover & QUBO & \color{red}{four classes of algorithmic approaches}& ? \\
numeric solver & Material deformation in production, tensil test  & FEM& high& medium& relevant & ? & &non-linear PDE's & differentiable quantum circuits & ? \\
process optimization & robot trajectory planning along which robots apply a PVC sealant along seams & ml? &high & medium & tolerant & 71 seams & travelling salesman & QUBO & QA & outperform greedy baseline results\\
%Preproduction & Pre-production vehicle configuration: MaxSAT  & real time & Cartypes: 25
%Features: 469 &  {\color{red}Algos with coherent Ising machines}/ Duerr–Høyer algorithm & No \\
%Quality control & Automated quality assessment: image recognition  & real time & \href {https://www.kaggle.com/datasets/arunrk7/surface-crack-detection}{40000}images with 227 x 227 pixels with RGB channels & QCNN: inner products, orthogonal matrix multiplication, multiplication in the fourier space & better trainability, faster convolution product in quantum simulation \\
 \multicolumn{6}{c}{\bf Airbus}\\\\
numeric solver &  accelerate linear solver of FVM (for shape aerodynamic optmization ) & Finite Volume Method & low & very high & tolerant & ? number of cells contained in the mesh & non-linear PDE's& linear equations & { \color{red} quantum linear solver } & ? \\
 desgin optimization &   reduce parameter space in wingbox optimisation & multistep (Laplace/Fourier transforms) & low & very high & tolerant & 6 structural parameters & binary classification (stress test) & QSVM (longterm HHL) & ? \\
 \multicolumn{6}{c}{\bf Deutsche Telekom}\\\\
 optimization & Mix sigma: combine allowence of relfelctor and lens to achieve a certain light reflection spec & none (matches unmeet spec would be trashed) & & high & low & relevant & 90 & ? combinatorical optimisation & QUBO & solved in less than a second with digital annealer
 \\
%   optimization&  machine assignment with the inclusion of automated guided vehicles & manual ? & high & real-time &four jobs, four machines
%and two AGVs (4x4x24x2) &JSSP & QUBO & QA & 
 %\multicolumn{6}{c}{\bf Bosch}\\\\
 %\multicolumn{6}{c}{\bf Siemens}\\\\
 
 %\multicolumn{6}{c}{\bf Aisin}\\\\
 %& vehicle routing &
 \multicolumn{6}{c}{\bf Trumpf}\\\\
 numericsolver  & tool modeling & FEM & medium & low & critical & 2000 matrix entries & non-linear PDE's & linear equations & HHL & ongoing research\\
  optimization & nesting and scheduling optimization in sheet metal processing & heuristics, manual & high & low & real-time & in the order of tousends & COP+JSSP & QUBO & QA & in progress \\

% \multicolumn{6}{c}{\bf Planerio}\\\\
 \bottomrule
 \caption{Your caption here} % needs to go inside
\label{tab:usecases}
  \end{longtable}
\end{landscape}
%\end{adjustbox}

